Spatially Resolved Physical Properties of Young Star Clusters and Star-forming Clumps in the Brightest z>6 Galaxy, the Strongly Lensed Cosmic Spear at z=6.2

We present spatially resolved analysis of stellar populations in the brightest $z>6$ galaxy known to date (AB mag 23), the strongly lensed MACS0308$-$zD1 (dubbed the ``Cosmic Spear'') at $z_{\rm spec}=6.2$. New JWST NIRCam imaging and high-resolution NIRSpec IFU spectroscopy span the rest-frame ultraviolet to optical. The NIRCam imaging reveals bright star-forming clumps and a tail consisting of three distinct, extremely compact star clusters that are multiply-imaged by gravitational lensing. The star clusters have delensed effective radii of $R_{\rm{eff}} \lesssim 8$ pc, stellar masses of $M_{*} \sim 10^{6}-10^{7}\,M_{\odot}$, and high stellar mass surface densities of $\Sigma_{*} \gtrsim 2\times 10^{4}\,M_{\odot}~\rm{pc}^{-2}$. While their stellar populations are very young ($\sim 6-11$ Myr), their dynamical ages exceed unity, consistent with the clusters being gravitationally bound systems. Placing the star clusters in the size vs.~stellar mass density plane, we find they occupy a region similar to other high-redshift star clusters within galaxies observed recently with JWST, being significantly more massive and denser than local star clusters. Spatially resolved analysis of the brightest clump reveals a compact, intensely star-forming core. The ionizing photon production efficiency ($\xi_{\rm{ion}}$) is slightly suppressed in this central region, potentially indicating a locally elevated Lyman continuum escape fraction facilitated by feedback-driven channels.

==> tbl_clumps_props1.tex <==
% Filters
\begin{deluxetable*}{lcccccccc}
\tablecaption{\label{tab:props_indiv_clumps}Measured Properties of the Clumps and Star Clusters in MACS0308$-z$D1
}
\tablewidth{\columnwidth}
\tablehead{
\colhead{ID} &
\colhead{$R_{\rm eff,obs}^{a}$} &
%\colhead{$R_{\rm eff,obs}} &
\colhead{$R_{\rm eff,int}^{b}$} &
\colhead{$M_{*,\rm{obs}}$} &
\colhead{$M_{*,\rm{int}}$} &
\colhead{$\Sigma_{*,\rm{int}}$} &
\colhead{Age$^{c}$} &
\colhead{$\Pi$} &
\colhead{$\mu_{\rm total}$}
\vspace{-0.07in}\\
\colhead{} &
\colhead{(pix)} &
%\colhead{(pc)} &
\colhead{(pc)} &
\colhead{($10^{7}\,$\Msun)} &
\colhead{($10^{7}\,$\Msun)} &
\colhead{($10^{3}\,$\sigmaMsunpc)} &
\colhead{(Myr)} &
\colhead{} &
\colhead{}
}
\startdata
%% intrinsic stellar masses are not corrected
% ID=3
$3a$
& $0.5 \pm 0.1$
& $5.9 \pm 0.1$
& ${9.1}_{-5.4}^{+6.4}$
& ${0.6}_{-0.4}^{+0.5}$
& ${16.6}_{-9.9}^{+11.9}$
& ${4.9}_{-1.6}^{+2.8}$
& ${5.8}_{-3.3}^{+6.2}$
& 14 \\
% ID=6
$3b$
& $0.9 \pm 0.04$
& $13.2 \pm 0.6$
& ${41.8}_{-23.7}^{+41.2}$
& ${3.8}_{-2.2}^{+3.7}$
& ${19.6}_{-11.9}^{+23.2}$
& ${11.8}_{-4.9}^{+13.6}$
& ${10.2}_{-6.6}^{+23.0}$
& 11 \\
% ID=7
$3c$
& $1.2 \pm 0.04$
& $15.1 \pm 0.5$
& ${10.0}_{-4.5}^{+5.3}$
& ${0.8}_{-0.3}^{+0.4}$
& ${3.0}_{-1.5}^{+1.9}$
& ${3.8}_{-1.7}^{+1.3}$
& ${1.2}_{-0.7}^{+0.9}$
& 13 \\
% ID=4
$4a$
& $0.9 \pm 0.01$
& $5.8 \pm 0.1$
& ${10.1}_{-5.6}^{+30.8}$
& ${0.4}_{-0.2}^{+1.2}$
& ${10.7}_{-6.0}^{+33.3}$
& ${5.5}_{-1.5}^{+14.6}$
& ${5.3}_{-2.7}^{+34.0}$
& 25 \\
% ID=5
$4b$
& $0.8 \pm 0.00$
& $5.3 \pm 0.0$
& ${5.4}_{-2.0}^{+5.3}$
& ${0.2}_{-0.1}^{+0.2}$
& ${6.8}_{-2.5}^{+6.7}$
& ${4.2}_{-1.4}^{+1.3}$
& ${3.4}_{-1.6}^{+2.8}$
& 25 \\
% ID=8
$5b$
& $1.0 \pm 0.00$
& $6.8 \pm 0.0$
& ${35.4}_{-18.1}^{+19.2}$
& ${1.4}_{-0.7}^{+0.8}$
& ${27.2}_{-13.9}^{+14.8}$
& ${17.0}_{-9.3}^{+13.0}$
& ${24.0}_{-16.4}^{+28.8}$
& 25 \\
% ID=9
$5c$
& $0.8 \pm 0.00$
& $5.4 \pm 0.0$
& ${13.3}_{-7.4}^{+15.3}$
& ${0.5}_{-0.3}^{+0.6}$
& ${16.3}_{-9.1}^{+18.8}$
& ${6.5}_{-2.1}^{+6.2}$
& ${8.1}_{-4.4}^{+14.9}$
& 25
\enddata
\tablenotetext{a}{PSF-deconvolved effective radius measured from F150W image using \galfit. The image has spatial sampling of $0\farcs04$ pixel$^{-1}$ and PSF FWHM of $0\farcs05$.}
\tablenotetext{b}{Intrinsic effective radius corrected for lensing tangential magnification (\mutan).}
\tablenotetext{c}{Fiducial age obtained from SED fitting using \piXedfit.}
\end{deluxetable*}


